Man and machine thinking about the smooth 4-dimensional Poincar\'e conjecture

While topologists have had possession of possible counterexamples to the smooth 4-dimensional Poincar\'{e} conjecture (SPC4) for over 30 years, until recently no invariant has existed which could potentially distinguish these examples from the standard 4-sphere. Rasmussen's s-invariant, a slice obstruction within the general framework of Khovanov homology, changes this state of affairs. We studied a class of knots K for which nonzero s(K) would yield a counterexample to SPC4. Computations are extremely costly and we had only completed two tests for those K, with the computations showing that s was 0, when a landmark posting of Akbulut (arXiv:0907.0136) altered the terrain. His posting, appearing only six days after our initial posting, proved that the family of ``Cappell--Shaneson'' homotopy spheres that we had geared up to study were in fact all standard. The method we describe remains viable but will have to be applied to other examples. Akbulut's work makes SPC4 seem more plausible, and in another section of this paper we explain that SPC4 is equivalent to an appropriate generalization of Property R (``in S^3, only an unknot can yield S^1 x S^2 under surgery''). We hope that this observation, and the rich relations between Property R and ideas such as taut foliations, contact geometry, and Heegaard Floer homology, will encourage 3-manifold topologists to look at SPC4.

==> todolist.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.


==> xypdf-c.tex <==
%% xypdf-c.tex from $Id: xypdf-c.doc,v $
%%
%% Xy-pic ``Colour extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-cloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-cloaded\endcsname=\empty \xycatcodes
\expandafter\ifx \csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\UsePDFcolor{\installPDFcolor@}
\xydef@\NoPDFcolor{\UnloadColor@}
\xydef@\installPDFcolor@{\installPDFstyle@
 \let\xymath@=\xyPDFmath@ \let\xynomath@=\xyPDFnomath@
 \let\checkxyPDFcolor@=\checkxyPDFcolor@@
 \let\xycolor@@=\xyPDFcolor@@
 \xystandardcolors@ 
 \xyuncatcodes }
\xydef@\xyPDFmath@{\hbox\bgroup\dimen@=.55ex \checkxyPDFcolor@ \xyinside@}
\xydef@\xyPDFnomath@{\hbox\bgroup\dimen@=\z@ \checkxyPDFcolor@ \xyinside@}
\xydef@\checkxyPDFcolor@@{\edef\pdfsaved@color{\pdfcurrent@color}%
 \let\checkxyPDFcolor@=\relax}
\xylet@\checkxyPDFcolor@=\relax
\xydef@\xyPDFnewcolor@#1#2#3#4#5{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@\newxycolor{#1}{}\relax\fi
 \DNii@{#4}\ifx\nextii@\empty
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPDFcolor@{#2//#3}}\else
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPDFcolor@{#4}}\fi
 \ifx\nextii@\empty\expandafter\def\next@{\xyPDFnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}\expandafter\tmp@\fi }
\xylet@\newxycolor@=\xyPDFnewcolor@
\xydef@\xyPDFcolor@{\ifPDFspecials@\expandafter\xyPDFcolor@@
 \else\expandafter\eat@\fi}
\xydef@\xyPDFcolor@@#1{\bgroup \checkXyStyle@ 
 \def\preStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPDFpre@}}%
 \def\postStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPDFpost@}}%
 \let\modPDFboxz@=\modXYstyle@ \xyPDF@color@@{#1}%
 \toks@={\egroup\let\xy@style@=\relax \def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \the\toks@ }

\xydef@\pdfcurrent@color{1 1 1 1 k 1 1 1 1 K}
\xydef@\pdfsaved@color{1 1 1 1 k 1 1 1 1 K}
\xydef@\xyPDF@color@@#1{%
 \edef\pdfsaved@color{\pdfcurrent@color}%
 \pdf@convertcolor#1////!%
 \edef\next@{\noexpand\xyPDFsplitPDF@{\pdfcurrent@color}{\pdfsaved@color}}%
 \next@}
\xydef@\pdf@convertcolor#1//#2//#3!{\DN@{#2}%
 \DNii@{cmyk}\ifx\next@\nextii@\DN@{#1 k #1 K}%
 \else \DNii@{rgb}\ifx\next@\nextii@\DN@{#1 rg #1 RG}%
 \else \DNii@{gray}\ifx\next@\nextii@\DN@{#1 #1 #1 rg #1 #1 #1 RG}%
 \else \DN@{1 1 1 1 k 1 1 1 1 K}%
 \fi \fi \fi 
 \expandafter\def\expandafter\pdfcurrent@color\expandafter{\next@}}
\xydef@\xycolor@raw@@#1{}%
\endinput


==> xypdf-f.tex <==
%% xypdf-f.tex from $Id: xypdf-f.doc,v $
%%
%% Xy-pic ``Frame extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-floaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-floaded\endcsname=\empty \xycatcodes
\xydef@\installPDFframes@{%
 \let\framed@body@@=\xyPDFframed@body@
 \let\circled@x@@=\xyPDFcircled@x@
 \let\ellipsed@x@@=\xyPDFellipsed@x@
 \installPDFfills@
 \xyuncatcodes}
\xydef@\UsePDFframes{\installPDFframes@}
\xydef@\NoPDFframes{\UnloadFrames@}
\xydef@\xyPDFframed@body@{\DN@{\framed@body@}%
 \ifx\framehfill\frm@solidh@@
 \DN@{\xyPDFframed@oval@\xyPDFoval@Special}%
 \else\ifdim\R@=\z@\else
 \ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFframed@oval@\xyPDFdashoval@Special}%
 \else\ifx\framehfill\frm@doth@@
 \DN@{\xyPDFframed@oval@\xyPDFdotoval@Special}%
 \fi\fi
 \fi\fi \next@ }
\xydef@\xyPDFframed@oval@#1{\vglue\U@c
 \hbox{\hglue\L@c\xypdfoval@#1\hglue\R@c}\vglue\D@c}
\xydef@\xyPDFcircled@x@{\DN@{\xyPDFcircled@x@@\xyPDFcirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPDFcircled@x@@\xyPDFdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFcircled@x@@\xyPDFdashcirc@Special}%
 \fi\fi \next@ }
\xydef@\xyPDFcircled@x@@#1{\vglue2\R@
 \hbox{\hglue2\R@\xypdfcircle@#1\hglue2\R@}%
 \vglue2\R@}
\xydef@\xyPDFellipsed@x@#1#2{%
 \DN@{\xyPDFellipsed@x@@\xyPDFcirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPDFellipsed@x@@\xyPDFdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPDFellipsed@x@@\xyPDFdashcirc@Special}%
 \fi\fi \next@{#1}{#2}}
\xydef@\xyPDFellipsed@x@@#1#2#3{\vglue #3\vglue #3\relax
 \hbox{\L@c = #2\relax \R@c=\L@c \D@c = #3\relax \U@c=\D@c 
 \hglue#2\hglue#2\relax\xypdfellipse@#1\hglue#2\hglue#2\relax}%
 \vglue #3\vglue #3\relax}
\xydef@\xyPDFdashhfill@{{\SemiDirectionChar=95 \Direction=3072 \xyPDFdash@}}
\xydef@\xyPDFdashvfill@{{\SemiDirection=31 \Direction=1023 \xyPDFdash@}}
\xydef@\xypdfoval@#1{%
 \dimen@=\L@c \advance\dimen@\R@c
 \dimen@ii=\U@c \advance\dimen@ii\D@c 
 \ifdim\dimen@ii<\dimen@ \relax \dimen@=\dimen@ii\fi \divide\dimen@\tw@
 \ifdim\R@>\dimen@ \relax \R@=\dimen@ \fi
 \D@c=-\D@c \L@c=-\L@c 
 \edef\tmp@{\expandafter\removePT@\the\R@
 \space\expandafter\removePT@\the\R@c 
 \space\expandafter\removePT@\the\D@c 
 \space\expandafter\removePT@\the\L@c 
 \space\expandafter\removePT@\the\U@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypdfcircle@#1{\dimen@=\R@
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypdfellipse@#1{\edef\tmp@{%
 \expandafter\removePT@\the\U@c \space
 \expandafter\removePT@\the\D@c \space
 \expandafter\removePT@\the\L@c \space
 \expandafter\removePT@\the\R@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xyPDFoval@Special#1{\PDFmacro@{#1 ov}}%%%%<<<---- here
\xydef@\xyPDFcirc@Special#1{\PDFmacro@{#1 ox}}%%%%<<<---- here
\xydef@\xyPDFdotcirc@Special#1{\PDFmacro@{#1 ot}}%%%%<<<---- here
\xydef@\xyPDFdashcirc@Special#1{\PDFmacro@{#1 od}}%%%%<<<---- here
\xydef@\xyPDFdotoval@Special#1{\PDFmacro@{#1 vt}}%%%%<<<---- here
\xydef@\xyPDFdashoval@Special#1{\PDFmacro@{#1 vd}}%%%%<<<---- here
\xydef@\xyPDFfilledRegion#1#2{\setboxz@h{\lower\D@c\vbox{%
 \vglue\U@c\hbox{#1#2\empty\hglue\L@c\hglue\R@c}\vglue\D@c}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\filledRectangle@PDF{%
 \xyPDFfilledRegion{\xypdfoval@\xyPDFfilloval@Special}}
\xydef@\filledCircle@PDF#1{{\R@c=\R@ \L@c=\R@ \U@c=\R@ \D@c=\R@
 \xyPDFfilledRegion{\xypdfcircle@\xyPDFfillcirc@Special}#1}}
\xydef@\filledEllipse@PDF{%
 \xyPDFfilledRegion{\xypdfellipse@\xyPDFfillellipse@Special}}
\xydef@\filledOval@PDF{%
 \xyPDFfilledRegion{\xypdfoval@\xyPDFfilloval@Special}}
\xydef@\frame@emph@PDF#1{\filled@{#1}\relax}
\xydef@\installPDFfills@{%
 \let\frame@emph@@=\frame@emph@PDF
 \let\filledRectangle@@=\filledRectangle@PDF
 \let\filledOval@@=\filledOval@PDF
 \let\filledCircle@@=\filledCircle@PDF
 \let\filledEllipse@@=\filledEllipse@PDF
}
\xydef@\xyPDFfilloval@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfo}%%%%%<<<---- here
 \else\PDFmacro@{#1 fo}\fi}%%%%<<<---- here
\xydef@\xyPDFfillcirc@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfc}%%%%%<<<---- here
 \else\PDFmacro@{#1 fc}\fi}%%%%<<<---- here
\xydef@\xyPDFfillellipse@Special#1#2{%
 \ifx#2\relax\PDFmacro@{#1 sfe}%%%%%<<<---- here
 \else\PDFmacro@{#1 fe}\fi}%%%%<<<---- here
\endinput


==> xypdf-l.tex <==
%% xypdf-l.tex from $Id: xypdf-l.doc,v $
%%
%% Xy-pic ``Line extension'' PDF backend support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-lloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-lloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\installPDFline@{\installPDFstyle@
 \installPDFlinestyles@ \installPDFpolylines@ }
\xydef@\UsePDFlines{\installPDFline@}
\xydef@\NoPDFlines{\UnloadLine@\relax}
\xydef@\xyPDFlineSpecial@#1{\xyPDFrawZ@{ #1 w}}
\xydef@\xyPDFcapSpecial@#1{\xyPDFrawZ@{ #1 J}}
\xydef@\xyPDFjoinSpecial@#1{\xyPDFrawZ@{ #1 j}}
\xydef@\xyPDFmiterSpecial@#1{\xyPDFrawZ@{ #1 M}}
\xydef@\installPDFlinestyles@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\transxyline@@=\transxyline@
 \let\xylineSpecial@@=\xyPDFlineSpecial@
 \let\resetxyline@@=\resetxyline@i
 \let\xy@linecap@@=\xy@linecap@
 \let\xycapSpecial@@=\xyPDFcapSpecial@
 \let\resetxylinecap@@=\resetxylinecap@i
 \let\xy@linejoin@@=\xy@linejoin@
 \let\xyjoinSpecial@@=\xyPDFjoinSpecial@
 \let\resetxylinejoin@@=\resetxylinejoin@i
 \let\xy@linemiter@@=\xy@linemiter@
 \let\xymiterSpecial@@=\xyPDFmiterSpecial@
 \let\resetxylinemiter@@=\resetxylinemiter@i
}
\xydef@\xypolylinePDF@Special#1{\PDFspecial@@{ q [] 0 d #1 S Q}}
\xydef@\xypolydotPDF@Special#1{\PDFspecial@@{ q [1 3] 0 d S Q}}
\xydef@\xypolydashPDF@Special#1{\PDFspecial@@{ q [5] 0 d #1 S Q}}
\xydef@\xypolyfillPDF@Special#1{\PDFspecial@@{ q #1 f Q}}
\xydef@\xypolyeofillPDF@Special#1{\PDFmacro@{ q #1 f* Q}}
\xydef@\installPDFpolylines@{%
 \let\xypolyline@Special=\xypolylinePDF@Special
 \let\xypolydot@Special=\xypolydotPDF@Special
 \let\xypolydash@Special=\xypolydashPDF@Special
 \let\xypolyfill@Special=\xypolyfillPDF@Special
%\let\xypolyeofill@Special=\xypolyeofillPDF@Special
 \let\xy@polystyle@@=\xy@polystyle@ }
\endinput


==> xypdf-r.tex <==
%% xypdf-r.tex from $Id: xypdf-r.doc,v $
%%
%% Xy-pic ``PDF Rotations and Scaling''.
%% Copyright (c) 1999-1999 Ross Moore <ross@maths.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-rloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-rloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty\else
 \xyinputorelse@{xypdf-s}{\xyerror@{Could not load xypdf-s}{}}%
 \xycatcodes\fi
\xydef@\installPDFrotscale@{\installPDFstyle@
% \let\xyRotate@@=\xyPDFrotate@@
% \let\doSpecialRotate@@=\doPDFspecialRotate@@
 \let\xyscale@@=\xyPDFscale@@
 \xyPDFshapes@true
 \xyuncatcodes }
\xydef@\UsePDFrotate{\installPDFrotscale@}
\xydef@\NoPDFrotate{\UnloadRotate@\relax}
\xydef@\xyPDFpretransform@{\xyPDFrawA@{\preXYtransform@@}}
\xydef@\xyPDFposttransform@{\xyPDFrawZ@{\postXYtransform@@}}
\let\preXYtransform@=\xyPDFpretransform@
\let\postXYtransform@=\xyPDFposttransform@
\xydef@\xyPDFrotSplit@{%
 \expandafter\def\expandafter\preShape@@\expandafter{\xyPDFpre@}%
 \expandafter\def\expandafter\postShape@@\expandafter{\xyPDFpost@}}
\xydef@\xyPDFscale@@#1#2{%
 \xyPDFsplitPDF@{\xyscale@start(#1,#2)}{\xyscale@end}%
 \xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\xyPDFrotate@@#1{%
 \xyPDFsplitPDF@{\xyrot@start(#1 xyd)}{\xyrot@end}%%%<<------ here
 \xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\xyPDFspecialRotate@#1{%
 \xyPDFsplitPDF@{\xyrot@start(#1)}{\xyrot@end}\xyPDFrotSplit@\xyPDFpdfxy@ }
\xydef@\doPDFspecialRotate@@#1@@{\xyPDFspecialRotate@{#1}}
\xydef@\xyRotScale@@{%
% \def\xyrot@start(##1){{xyt ##1\space xyr}}%%%<<------ here
 \def\xyscale@start(##1,##2){ q ##1 0 0 ##2 0 0 cm}%
 \def\xyrot@end{ Q}\def\xyscale@end{ Q}}
\endinput


==> xypdf-s.tex <==
%% xypdf-s.tex from $Id: xypdf-s.doc,v $
%%
%% Xy-pic ``Style extension'' PDF support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-sloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-sloaded\endcsname=\empty \xycatcodes
\xydef@\xykillstyles@@{\Unloadstyle@}%
\xywarnifdefined\xyPDFescapestyle@
\xywarnifdefined\xyPDFsplitescape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPDFescapestyle@#1@@{\xyPDFsplitescape@#1<><>@@}%
 \gdef\xyPDFsplitescape@#1<>#2<>#3@@{\xyescape@@{#1}{#2}}}
\xydef@\xyPDFsplitPDF@#1#2{%
 \def\xyPDFpre@{#1}\def\xyPDFpost@{#2}\modPDFboxz@ }
\xydef@\xyescape@@#1#2{\checkXyStyle@ 
 \applyFIFOstyle@\prexyescape@{#1}\postxyescape@{#2}}
\xydef@\prexyescape@{\xyescapeSpecial@}
\xydef@\postxyescape@{\xyescapeSpecial@}
\xylet@\xyescapeSpecial@=\eat@
\let\xyescapeSpecial@=\addtostyletoks@
\xydef@\installPDFstyle@{%
 \def\preXYstyle@@{\xyPDFpre@}%
 \let\xydoprestyles@=\xyPDFrawstyleA@
 \let\xydopoststyles@=\xyPDFrawZ@
 \let\xykillstyles@=\xykillstyles@@
 }
\xydef@\xyPDFrawstyleA@#1{\xyPDFrawA@{{#1}{}}}
\endinput


==> xypdfpdf.tex <==
%% xypdfpdf.tex from $Id: xypdfpdf.doc,v $
%%
%% Xy-pic ``PDF-PDF'' PDF support.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xypdf-pdfloaded\endcsname=\empty \xycatcodes
\global\newif\ifPDFspecials@
\xylet@\PDFmacro@@=\eat@
\xylet@\PDFdict@@=\eat@
\xylet@\PDFspecial@@=\eat@
\xylet@\PDFread@@=\eat@
\xylet@\PDFinclude@@=\eat@
\xylet@\PDFraw@@=\eat@
\xylet@\xyPDFobeylines@@=\relax
\xylet@\PDFspecialdict@@=\eat@
\xydef@\UnloadPDFpdf@{%
 \let\PDFmacro@@=\eat@
 \let\PDFdict@@=\eat@
 \let\PDFspecial@@=\eat@
 \let\PDFread@@=\eat@
 \let\PDFinclude@@=\eat@
 \let\PDFraw@@=\eat@
 \let\xyPDFobeylines@@=\relax
 \let\PDFspecialdict@@=\eat@
}
\xydef@\UnloadPDF@{\UnloadPDFpdf@
 \expandafter\ifx\csname xypdfloaded\endcsname\unknown\PDFspecials@false
 \else\expandafter\NoPDFspecials\fi}
\xylet@\UnloadPDF@@=\UnloadPDF@
\ifx\undefined\dvitype@\xydef@\dvitype@{null}\fi
\xylet@\xyrealshipout@=\shipout
\xydef@\xyPDFshipout@{\xyrealshipout@}
\xydef@\firstPDF@{%
 \global\let\firstPDF@@=\relax \global\let\firstPDF@=\relax}
\xylet@\firstPDF@@=\firstPDF@
\xylet@\dumpPDFdict@@=\relax
\xydef@\installxypdf@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}\xycatcodes
 \installxypdf@@ \installxypdf@x }
\xylet@\installxypdf@@=\relax
\xylet@\setupxyPDF@@=\PDFspecials@true
\xywithoption{pdf}{\let\setupxyPDF@@=\setupxyPDF@}
\xydef@\installxypdf@x{
 \let\firstPDF@=\relax
 \let\XYpredict@=\relax
 \setupxyPDF@@ }
\xydef@\setupxyPDF@{\PDFspecials@true}
\let\realinstallxypdf@x=\installxypdf@x
\ifx\undefined\AfterBeginDocument
 \def\installxypdf@x{\xysetup@@{\realinstallxypdf@x}}%
\else
 \def\installxypdf@x{\AfterBeginDocument{\realinstallxypdf@x}}%
\fi
\xydef@\xydefaultdriver@{dvipdf}
\xydef@\xyPDFdriver#1{\def\xydefaultdriver@{#1}}
\xydef@\installxypdf@orig{\DN@{}%
 \ifx\xydriversselected@@\empty
 \DN@{\expandafter\defaultinstallpdf@\expandafter{\xydefaultdriver@}}%
 \else \def\do##1{%
 \expandafter\ifx\csname##1@xy@pdf\endcsname\relax
 \DN@{\defaultinstallpdf@{##1}}}%
 \xydriversselected@@ 
 \else \DN@##1{}\fi\fi \next@ }
\xydef@\defaultinstallpdf@#1#2{%
 \xywarning@{no driver specified, using #1 }%
 \xyrequire{#1}\csname #1@xy@pdf\endcsname{}}
\xydef@\null@xy@pdf{\installxypdf@}
\xydefcsname@{shape [!...]}#1{%
 \expandafter\ifx\csname xypdf-sloaded\endcsname\empty \DN@{\xyPDFescapestyle@{#1}@@}%
 \else\ifxyPDFshapes@\DN@{\xyPDFshapechar@{#1}@@}%
 \else \DN@{\xyPDFcharwarning@}\fi\fi \next@ }
\xydefcsname@{shape [pdfxy]}{\ifxyPDFshapes@\DN@{\xyPDFpdfxy@}%
 \else \DN@{\xyPDFcharwarning@}\fi \next@ }
\xydef@\xyPDFpdfxy@{%
 \setboxz@h{\dimen@=\L@p \advance\dimen@-\R@p 
 \dimen@ii=-\U@p \raise\dimen@ii\hbox to\z@{%
 \kern\dimen@\xyPDFcurrpt@\kern-\dimen@}\boxz@}}%
\xydef@\xyPDFcurrpt@{\ifxyPDFshapes@\expandafter\xyPDFcurrpt@@\fi}
\xydef@\xyPDFcurrpt@@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%<<<<<--- here
\ifx\undefined\xyPDFcurrpt@@ \xylet@\xyPDFcurrpt@@=\xyPDFcurrpt@@@ \fi
\xywarnifdefined\xyPDFshapechar@
\xywarnifdefined\xyPDFsplitshape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPDFshapechar@#1@@{\xyPDFsplitshape@#1<><>@@}%
 \gdef\xyPDFsplitshape@#1<>#2<>#3@@{\xyPDFsplitPDF@{#1}{#2}}}
\xydef@\xyPDFrawA@#1{\expandafter\xyPDFrawAA@ #1{}{}}%
\xydef@\xyPDFrawAA@#1#2{\PDFraw@@{ #1 #2}\PDFmessage{ #1 #2 }}%
\xydef@\xyPDFrawZ@#1{\PDFraw@@{ #1}\PDFmessage{ #1 }}%
\xydef@\modPDFboxz@{%
 \expandafter\DN@\expandafter{\xyPDFpre@{}}\ifx\next@\empty\else
 \setboxz@h{\expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}\boxz@
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}\DN@{}\fi}%
\xydef@\modPDFdrop@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Drop@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}%
 \DN@##1{\expandafter\def\expandafter\Drop@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\modPDFconnect@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawA@\expandafter{\xyPDFpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Connect@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPDFrawZ@\expandafter{\xyPDFpost@}}%
 \DN@##1{\expandafter\def\expandafter\Connect@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\xyPDFpre@{{}{}}
\xydef@\xyPDFpost@{}
\xydef@\PDFmessage@#1{\W@{PDF: #1}}
\xydef@\PDFignore@#1{}%
\xydef@\showPDFmessages{\let\PDFmessage=\PDFmessage@}
\xydef@\hidePDFmessages{\let\PDFmessage=\PDFignore@}
\xylet@\PDFtracing=\showPDFmessages
\hidePDFmessages
\xydef@\PDFmacro@#1{\PDFmacro@@{#1}\PDFmessage{#1}}
\xydef@\includeXYPDFdict@{\relax}
\xydef@\xyPDFdictknown@{}
\xywarnifdefined\obeyoutlines@
{\catcode`\^^M=\active%
 \gdef\obeyoutlines@{\catcode`\^^M=\active \def^^M{^^J}%
 \newlinechar=`\^^J\obeyspaces}}
\xynew@{if}\ifxyPDFshapes@ \xyPDFshapes@true 
\xydef@\xyPDFcharwarning@@{\xyPDFcharmessage@
 \gdef\xyPDFcharwarning@@{\xyPDFcharmessage@
 \xywarning@{...no further PDF warnings will be given}%
 \global\let\xyPDFcharwarning@@=\relax }}
\xydef@\xyPDFcharmessage@{\xywarning@{%
 the current <driver> does not fully support PDF effects}}%
\xydef@\newxyshape#1#2#3{%
 \DN@{#3}\ifx\next@\empty
 \xydefcsname@{shape [#1]}{\csname xyshape@#1@\endcsname}%
 \else \expandafter\def\csname shape [#1]\endcsname{%
 \csname xyshape@#1@\endcsname}\fi
 \DN@{#2}\ifx\next@\empty
 \expandafter\def\csname xyshape@#1@\endcsname{%
 \xyundefinedEffect@{#1}{}@@}%
 \else \expandafter\def\csname xyshape@#1@\endcsname{#2}\fi }
\xydef@\xyundefinedEffect@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver}}%
\xydef@\newxyPDFshape#1#2{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@ \newxyshape{#1}{}\relax\fi
 \expandafter\DNii@\expandafter{\csname xyPDFshape@#1@\endcsname}%
 \expandafter\def\nextii@{#2}%
 \ifx\nextii@\empty\expandafter\def\next@{\xyPDFnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}%
 \expandafter\tmp@\fi }
\xydef@\xyPDFnotimplemented@@#1@@{%
 \xywarning@{This PostScript effect is not implemented yet}}%
\xydef@\xyPDFnotfinished@@{%
 \xywarning@{This effect is not reliable yet; box sizes may be wrong}}%
\installxypdf@
\endinput








==> xypdftex.tex <==
%% xypdftex.tex from $Id: xypdftex.doc,v $
%%
%% Xy-pic ``pdf-TeX'' driver interface option.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{pdftex}{pdf-TeX driver}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\pdfTeX@@#1{\dvimessage@{pdf-TeX}{#1}}
\newdriver{%
 \xyaddsupport{color}\pdftexColor@@
 \xyaddsupport{crayon}\pdftexCrayon@@
% \xyaddsupport{pdf}\pdftexPDF@@
% \xyaddsupport{rotate}\pdftexRotate@@
 \xyaddsupport{line}\pdftexLine@@
% \xyaddsupport{frame}\pdftexFrames@@
% \xyaddsupport{tile}\pdftexTiles@@
 \xyaddsupport{cmtip}\relax
}
%\xydef@\pdfTeXcolor@push#1{\special{pdfcolor push}\special{pdfcolor #1}}
\xydef@\pdfTeXcolor@push#1{\edef\pdfsaved@color{\pdfcurrent@color}%
 \def\pdfcurrent@color{#1}\special{#1}}%%%<<<<<<--- WRONG !
\xydef@\pdfTeXcolor@pop{\let\pdfcurrent@color\pdfsaved@color
 \expandafter\special\expandafter{\pdfsaved@color}}
\xydef@\pdfTeXcolours@{\pdftexPDFtypes@
% \let\xylocalColor@=\xystackcolor@
% \let\xycolor@push=\pdfTeXcolor@push
% \let\xycolor@pop=\pdfTeXcolor@pop
 \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-c}{\xydrivernoload@{pdf-c}}%
 \if@pdf@known\installPDFcolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\pdftexCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@ 
 \let\xycolorwarning@=\relax \pdfTeX@@{color}%
 \let\pdftexColor@@=\relax
 \let\UnloadColor@@=\NopdfTeXcolor@
 }
\xydef@\pdftexColor@@{\pdfTeXcolours@}
\xydef@\NopdfTeXcolor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\pdftexColor@@=\pdfTeXcolours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\pdftexCrayon@@{\pdftexColor@@\pdftexCrayon@}
\xydef@\pdftexCrayon@{\installCrayolaColors@}%
\xydef@\pdftexPDF@@{\if@pdf@known\pdftexPDF@}
\xydef@\pdftexPDFunload@{\if@pdf@known\UnloadPDF@
 \let\UnloadPDF@@=\UnloadPDF@
 \let\pdftexPDF@@=\pdftexPDF@ }
\xydef@\pdftexPDFtypes@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}%
 \ifx\PDFspecial@@\pdfTeXspecial@\else
 \let\PDFspecial@@=\pdfTeXspecial@
 \let\PDFmacro@@=\pdfTeXmacro@
 \let\PDFdict@@=\pdfTeXdict@
 \let\PDFraw@@=\pdfTeXraw@
 \let\PDFinclude@@=\pdfTeXinclude@
 \let\PDFspecialdict@@=\pdfTeXspecialDict@
 \let\xyPDFobeylines@@=\obeypdfTeXlines@
 \pdfTeX@@{PDF}%
 \fi \pdftexCurrpt@ }
\xydef@\pdfTeXspecial@#1{\if@pdf@known\firstPDF@@\pdfobj{#1}\pdflastobj}
\xydef@\pdfTeXmacro@#1{\pdfobj{#1}}
\xydef@\pdfTeXdict@#1{\pdfnames{#1}}
\xydef@\pdfTeXspecialDict@#1{\pdfnames{#1}}
\xydef@\pdfTeXinclude@#1{\if@pdf@known\firstPDF@@\special{prePDFfile #1}}
\xydef@\pdfTeXraw@#1{\if@pdf@known\firstPDF@@\pdfliteral{#1}}%
{\catcode`\^^M=\active%
 \gdef\next{\catcode`\^^M=\active \let^^M=\par%
 \let\PDFspecial@@=\pdfTeXdict@ \obeyspaces}}
\xylet@\obeypdfTeXlines@=\next
\xydef@\pdftexCurrpt@{\let\xyPDFcurrpt@@=\pdftexCurrpt@@}%
\xydef@\pdftexCurrpt@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%%<<<<<--- here
\xydef@\pdftexPDF@{\pdftexPDFtypes@
 \let\pdftexPDF@@=\relax
 \let\UnloadPDF@@=\pdftexPDFunload@ 
 \let\installxypdf@@=\relax \if@pdf@known\installxypdf@ }
\xydef@\pdftexRotate@@{\pdftexRotate@}
\xydef@\pdftexRotate@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-r}{\xydrivernoload@{pdf-r}}%
 \xyRotScale@@ \if@pdf@known\installPDFrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\if@pdf@known\UnloadRotate@\relax}\fi
 \next@}
\xydef@\pdftexLine@@{\pdftexLine@}
\xydef@\pdftexLine@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-l}{\xydrivernoload@{pdf-l}}%
 \if@pdf@known\installPDFline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\if@pdf@known\UnloadLine@\relax}\fi
 \next@ }
\xydef@\pdftexFrames@@{\pdftexFrames@}
\xydef@\pdftexFrames@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-f}{\xydrivernoload@{pdf-f}}%
 \if@pdf@known\installPDFframes@ }%
 \else\DN@{\xydriverfail@{frames are}\if@pdf@known\UnloadPDFframes@\relax}\fi
 \next@ }
\xydef@\pdftexTiles@@{\pdftexTiles@}
\xydef@\pdftexTiles@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-t}{\xydrivernoload@{pdf-t}}%
 \if@pdf@known\installPDFpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\if@pdf@known\UnloadPDFpatterns@\relax}\fi
 \next@ }
\xydef@\if@pdf@known#1{\ifx\undefined#1\else\expandafter#1\fi}
\xyendinput



